D2M: A Decentralized, Privacy-Preserving, Incentive-Compatible Data Marketplace for Collaborative Learning

The rising demand for collaborative machine learning and data analytics calls for secure and decentralized data sharing frameworks that balance privacy, trust, and incentives. Existing approaches, including federated learning (FL) and blockchain-based data markets, fall short: FL often depends on trusted aggregators and lacks Byzantine robustness, while blockchain frameworks struggle with computation-intensive training and incentive integration. We present \prot, a decentralized data marketplace that unifies federated learning, blockchain arbitration, and economic incentives into a single framework for privacy-preserving data sharing. \prot\ enables data buyers to submit bid-based requests via blockchain smart contracts, which manage auctions, escrow, and dispute resolution. Computationally intensive training is delegated to \cone\ (\uline{Co}mpute \uline{N}etwork for \uline{E}xecution), an off-chain distributed execution layer. To safeguard against adversarial behavior, \prot\ integrates a modified YODA protocol with exponentially growing execution sets for resilient consensus, and introduces Corrected OSMD to mitigate malicious or low-quality contributions from sellers. All protocols are incentive-compatible, and our game-theoretic analysis establishes honesty as the dominant strategy. We implement \prot\ on Ethereum and evaluate it over benchmark datasets -- MNIST, Fashion-MNIST, and CIFAR-10 -- under varying adversarial settings. \prot\ achieves up to 99\% accuracy on MNIST and 90\% on Fashion-MNIST, with less than 3\% degradation up to 30\% Byzantine nodes, and 56\% accuracy on CIFAR-10 despite its complexity. Our results show that \prot\ ensures privacy, maintains robustness under adversarial conditions, and scales efficiently with the number of participants, making it a practical foundation for real-world decentralized data sharing.

==> sections/YashAndShlinInput.tex <==
% Yash's part
% I will explain D2M Core algorithm (Algorithm 2 below)
% \subsection{\prot\ Core}
% \label{sec:core}
% After the on‐chain auction identifies the winning bid
% \[
%   R^*=\{\xi,\;Amt,\;\mathcal{K},\;M,\;\tau\}
% \]
% and matches it with dataset sellers \(\mathcal{S}\), the \prot\ Core protocol (Algorithm~\ref{alg:workflow}) executes off‐chain. Its goal is to produce a final model \(\widehat{\mathcal{K}}\) while ensuring:
% \begin{itemize}
%   \item \textbf{Byzantine Resilience}: tolerate up to \(f_{\max}\) malicious compute nodes or sellers,
%   \item \textbf{Efficiency}: minimize communication rounds and computation cost,
%   \item \textbf{Fairness}: reward each participant exactly in proportion to its verified contribution.
% \end{itemize}

% \paragraph{Notation.}
% \begin{itemize}
%   \item \(R^*=\{\xi,Amt,\mathcal{K},M,\tau\}\): winning bid request—\(\xi\) are data‐tags, \(Amt\) is total payment, \(\mathcal{K}\) is the initial model, \(M\) is the metric, \(\tau\) is the performance target.
%   \item \(\mathcal{S}\): set of sellers with matching data.
%   \item \(t_{\max}\): maximum allowed global rounds.
%   \item \(w^t\): global model weights in round \(t\).
%   \item \(p^t\): sampling probabilities over \(\mathcal{S}\) in round \(t\).
%   \item \(N^t\): cumulative seller‐contribution vector in round \(t\).
%   \item \(NC\): cumulative compute‐node participation counters.
%   \item \(\theta\): likelihood threshold for consensus.
%   \item \(ES_i\): Execution Set in mini‐round \(i\).
%   \item \(L_{k,i}\): likelihood score of digest \(k\) after mini‐round \(i\).
%   \item \(\widehat{\mathcal{K}},\widehat{N},\widehat{NC}\): final outputs.
% \end{itemize}

% \begin{algorithm}[H]
% \caption{\prot\ Core Algorithm}
% \label{alg:workflow}
% \begin{algorithmic}[1]
% \State \textbf{Input:} \(R^*,\,\mathcal{S},\,t_{\max}\)
% \State \textbf{Output:} \(\widehat{\mathcal{K}},\,\widehat{N},\,\widehat{NC}\)
% \State Initialize:
% \[
%   t\leftarrow0,\;
%   w^0\leftarrow\mathcal{K},\;
%   p^0\leftarrow\tfrac{1}{|\mathcal{S}|}\mathbf1,\;
%   N^0\leftarrow\mathbf0,\;
%   NC\leftarrow\mathbf0.
% \]
% \While{\(M(w^t)<\tau\) \textbf{and} \(t<t_{\max}\)}
%   \State \(i\leftarrow0\); \(k\leftarrow 0 ; L_{0,0}\leftarrow0\)
%   \While{\(\forall k:\;L_{k,i}\le\theta\)}
%     \State \(i\leftarrow i+1\)
%     \State \(ES_i\leftarrow\text{YODA sortition(size}=\mathit{base}+2^{i-1})\)
%     \ForAll{\(j\in ES_i\)}
%       \State \(NC[j]\mathrel{+}=1\)
%       \State \(\{w^t_{i,j},p^t_{i,j},N^t_{i,j}\}\leftarrow\) Algorithm~\ref{alg:osmd}\((w^t,p^t)\)
%       \State Commit \(H(w^t_{i,j},p^t_{i,j},N^t_{i,j})\) on‐chain
%     \EndFor
%     \ForAll{digest \(k\)}
%       \State \(L_{k,i}\leftarrow\sum_{l=1}^i (2\,c_{k,l}-C_l)\,C_l\),\\
%       where \(c_{k,l}\) = \# nodes in \(ES_l\) with hash \(k\), \(C_l=|ES_l|\)
%     \EndFor
%   \EndWhile
%   \State Select \(k'\) with \(L_{k',i}>\theta\)
%   \State \((w^{t+1},p^{t+1},N^{t+1})\leftarrow(w^t_{i,k'},p^t_{i,k'},N^t_{i,k'})\)
%   \State \(t\leftarrow t+1\)
% \EndWhile
% \State \(\widehat{\mathcal{K}}\leftarrow w^t,\;\widehat{N}\leftarrow N^t,\;\widehat{NC}\leftarrow NC\)
% \end{algorithmic}
% \end{algorithm}

% \paragraph{Detailed Rationale.}  
% We begin by initializing the round counter \(t\), model weights \(w^0\), uniform seller probabilities \(p^0\), and zeroed contribution counters \(N^0,NC\).  This creates a neutral starting state with no bias.

% The \textbf{outer loop} continues until the model’s performance \(M(w^t)\) meets the buyer’s target \(\tau\) or we exhaust \(t_{\max}\) rounds—this bounds cost while striving for required quality.

% At the start of each global round, we initialize a mini‐round index \(i=0\) and reset all likelihood scores \(L_{k,0}=0\).  These scores will measure how strongly compute nodes agree on each candidate update.

% Within the \textbf{inner loop}, we increment \(i\) and form an Execution Set \(ES_i\) of size \(\mathit{size}_{i-1}+2^{i-1}\).  By starting small and doubling, we minimize communication when nodes quickly agree, yet guarantee an honest majority will eventually dominate even if some nodes are malicious.

% Each node \(j\in ES_i\) logs its participation \(NC[j]\mathrel{{+}{=}}1\) for fair compute‐reward accounting, then runs the Corrected OSMD routine on \((w^t,p^t)\).  Corrected OSMD (detailed in Section~\ref{sec:osmd}) adaptively selects high‐value sellers, combines their updates into candidate weights \(w^t_{i,j}\), revises sampling probabilities \(p^t_{i,j}\), and updates per‐seller contributions \(N^t_{i,j}\).  The node then commits a cryptographic hash \(H(\cdot)\) of its result on‐chain, preventing any post‐hoc change and enabling verifiable audit.

% To decide which candidate update to accept, we compute for each digest \(k\) the \emph{likelihood score}
% \[
%   L_{k,i} = \sum_{l=1}^i (2\,c_{k,l} - C_l)\,C_l,
% \]
% where \(c_{k,l}\) counts how many nodes in mini‐round \(l\) produced hash \(k\), and \(C_l\) is the ES size.  This score grows rapidly when many independent nodes agree, providing a clear statistical signal.  We compare \(L_{k,i}\) against a precomputed threshold
% \[
%   \theta = \Bigl(\ln\tfrac{1-\beta}{\beta}\Bigr)\,
%   \frac{2\,q(1-q)\,C\,(1-f_{\max})\,f_{\max}}{(1-f_{\max})-f_{\max}},
% \]
% derived to balance \emph{speed} (fewer mini‐rounds) with \emph{security} (rejecting Byzantine proposals). It is derived from:
% \begin{itemize}
%     \item Desired statistical confidence level (\(1 - \beta\)).
%     \item Number of \cone\ nodes \(C\).
%     \item Fraction \(q\) of \cone\ selected per round in the ES.
%     \item Assumed upper bound \(f_{\text{max}}\) on the fraction of byzantine nodes.
% \end{itemize}

% \[
% \theta \gets \left(\ln \frac{1 - \beta}{\beta}\right) 
% \cdot \frac{2q(1 - q)C(1 - f_{\text{max}})f_{\text{max}}}{(1 - f_{\text{max}}) - f_{\text{max}}}
% \]  If no \(L_{k,i}>\theta\), we repeat with a larger ES.

% Once some \(k'\) satisfies \(L_{k',i}>\theta\), we accept and adopt its corresponding update:
% \[
%   (w^{t+1},\,p^{t+1},\,N^{t+1}) 
%   \;=\;(w^t_{i,k'},\,p^t_{i,k'},\,N^t_{i,k'}).
% \]
% This reflects the candidate with the strongest, independent support.  We increment \(t\) and repeat, steadily improving the model.

% Finally, when performance \(M(w^t)\ge\tau\) or \(t=t_{\max}\), we output the trained model \(\widehat{\mathcal{K}}=w^t\), the seller contributions \(\widehat{N}=N^t\), and compute‐node counts \(\widehat{NC}=NC\).  These values feed back to the on‐chain contract for precise, fair distribution of the payment \(Amt\).

% By uniting YODA’s efficient, random node selection, MIRACLE’s rigorous likelihood‐based consensus, and OSMD’s utility‐driven sampling, \prot\ Core achieves the target \(\tau\) with minimal rounds, provable Byzantine tolerance, and exact fairness in rewards.  


% Shalin's part
% I will explain the Corrected OSMD Sampler and Aggregator Alogrithm below
\subsection{Corrected OSMD}
\label{sec:osmd}

Corrected OSMD Sampler and Aggregator is an algorithm designed to improve a machine learning model by intelligently selecting and aggregating updates from multiple data sellers. We know that all sellers are not equally useful and some might send malicious updates and we also want to be fair and efficient in choosing from whom we want updates. So we use Corrected OSMD as strategy to learn which sellers are most helpful over time.

In any round $t$ of the D2M core algorithm we have following as our inputs for Algorithm 3.
\begin{itemize}
    \item Model parameters (weights) $w^{t}$ that we want to update.
    \item A probability distribution $p^t$, which tells us how likely we are to pick each seller.
    \item A record of how many times each dataset has been asked before denoted by $N^t$.
    \item Some settings required to run the algorithm are as follows: 
        \begin{itemize}
            \item $K:$ Number of sellers to be sampled in this round.
            \item $\eta:$ Learning rate, how fast we want to update the weights.
            \item $\gamma_t:$ Step size, how big of a change in updates we allow in each round.
            \item $\alpha:$ Controls fairness - everyone gets atleast a chance to get sampled.
        \end{itemize}
\end{itemize}

In each round, we randomly select $K$ sellers based on the probabilities in $p^t$. These sellers receive the current model and return their proposed updates, based on their own private data. We record which sellers were selected and update their access counts in $N^{t+1}$. For each seller, we then calculate how helpful their update was—the algorithm computes the gradient-based vector $\widehat{u}^t$, where each component $\widehat{u}_i^t$ is defined as:
\[
\widehat{u}_i^t = \frac{\sum_{k=0}^{K-1} \mathds{1}\{i^{t,k} = i\}}{K p_i^t} \times \big(U(w^t + \gamma_t g_i^t) - U(w^t)\big),
\]
where $\mathds{1}\{i^{t,k} = i\}$ is an indicator function that counts the occurrences of provider $i$ in the sampled batch. The term $U(w^t + \gamma_t g_i^t) - U(w^t)$ represents the utility difference due to the model update. The scaling factor accounts for the sampling probability $p_i^t$ and ensures unbiased estimation (Line 8).

Next, using these utility scores, we update the sampling distribution $p^t$. To update $p^t$ we solve the following optimization problem: \[
       p^{t+1} \;=\;
       \arg\min_{q\in\mathcal{A}}
         \bigl\langle q,\widehat u^t\bigr\rangle
         +D_\Phi(q\|p^t)
     \]
This formulation balances exploitation (preferring sellers with low estimated utility values, which indicate high contributions) and exploration (not deviating too far from the previous distribution 
$p^t$). The term $\bigl\langle q,\widehat u^t\bigr\rangle$ encourages selecting more helpful sellers, while the Bregman divergence $D_\Phi(q\|p^t)$ regularizes the change in distribution to maintain stability and fairness.

The update is computed using the Online Mirror Descent (OMD) solver. For a detailed derivation and theoretical guarantees of OMD solver, we refer the reader to the original paper \cite{ZhaoOSMD}(Line 9).

Finally instead of simply averaging the updates (which could be affected by malicious or noisy inputs) we use a robust method called Corrected KRUM which selects the single update closest to the mean among the refined subset, mitigating the influence of Byzantine sellers and produce the updated model parameters $w^{t+1}$. This ensured that only the most reliable updates are used, leading to a more accurate and secure learning process over time.

For a detailed overview of Corrected KRUM. we refer the reader to the original paper\cite{DuBlockchainDML}.

\begin{algorithm}[tbp]
\caption{Corrected OSMD Sampler and Aggregator}
\label{alg:osmd}
\begin{algorithmic}[1]
   \State \textbf{Input:}
      \begin{itemize}
   \item round $t$, batch size $K$
       \item OSMD learning rate $\eta$ 
       \item optimization stepsizes $\{\gamma_t\}_{t=0}^{T-1}$
       \item parameter $\alpha \in [0,1]$, $\mathcal{A} = \mathcal{P}_{n-1} \cap [\alpha/n, \infty)^n$
       \item the sampling distribution $p^t$ and model parameter $w^t$.
       \item the number of accesses for each dataset $N^t$
   \end{itemize}
   \State \textbf{Output:} 
   \begin{itemize}
       \item trained model's parameters $w^{t+1}$
       \item number of accesses for each seller $N^{t+1}(i) \ \forall \ i \in [n]$
       \item sampling distribution $p^{t+1}$
   \end{itemize}
   \State Sample \(K\) sellers \(S^t=\{i^{t,0},\dots,i^{t,K-1}\}\) with replacement from \(p^t\).
   \ForAll{\(i\in S^t\)} 
     \State Send \(w^t\) to seller \(i\); receive update \(g_i^t=\mathcal{O}_i(w^t)\).
   \EndFor
   \State Update counts: 
     \(N^{t+1}(i)=N^t(i)+\sum_k\mathbf{1}\{i^{t,k}=i\}\).
   \State Compute utility estimates
     \[
       \widehat u_i^t
       =\frac{\sum_k\mathds{1}\{i^{t,k}=i\}}{K\,p_i^t}
        \bigl[\,U(w^t+\gamma_t\,g_i^t)-U(w^t)\bigr].
     \]
   \State Solve for new sampling distribution
     \[
       p^{t+1} \;=\;
       \arg\min_{q\in\mathcal{A}}
         \bigl\langle q,\widehat u^t\bigr\rangle
         +D_\Phi(q\|p^t)
     \]
     via the OMD solver \cite{ZhaoOSMD}.
   \State Aggregate model updates with Corrected Krum \cite{DuBlockchainDML}:
     \[
       w^{t+1}
       \;=\;\text{Krum}\bigl\{\,w^t+\gamma_t\,g_i^t\,:\,i\in S^t\}\,.
     \]
\end{algorithmic}
\end{algorithm}
